Leveraging Experience in Lifelong Multi-Agent Pathfinding

In Lifelong Multi-Agent Path Finding (L-MAPF) a team of agents performs a stream of tasks consisting of multiple locations to be visited by the agents on a shared graph while avoiding collisions with one another. L-MAPF is typically tackled by partitioning it into multiple consecutive, and hence similar, "one-shot" MAPF queries, as in the Rolling-Horizon Collision Resolution (RHCR) algorithm. Therefore, a solution to one query informs the next query, which leads to similarity with respect to the agents' start and goal positions, and how collisions need to be resolved from one query to the next. Thus, experience from solving one MAPF query can potentially be used to speedup solving the next one. Despite this intuition, current L-MAPF planners solve consecutive MAPF queries from scratch. In this paper, we introduce a new RHCR-inspired approach called exRHCR, which exploits experience in its constituent MAPF queries. In particular, exRHCR employs an extension of Priority-Based Search (PBS), a state-of-the-art MAPF solver. The extension, which we call exPBS, allows to warm-start the search with the priorities between agents used by PBS in the previous MAPF instances. We demonstrate empirically that exRHCR solves L-MAPF instances up to 39% faster than RHCR, and has the potential to increase system throughput for given task streams by increasing the number of agents a planner can cope with for a given time budget.

==> tex/future_work.tex <==

\section{Future Work}\label{sec:future_work}
Our algorithmic framework suggests an improvement for the MAPF and the L-MAPF problems address several sub-problems.
We focused on proof of concepts and improving a state-of-the-art algorithm, which is known as a fast one and is applicable for real-world scenarios.
Accordingly, future work can be done to improve our first solutions. 

\paragraph{Offline and artificial experience}
We used an online gained experience, but, it is also possible to create an \quot{experience database} that contains queries and their solution priorities, and retrieve the nearest neighbor under some metric to be used in \expbs.
Additionally, it is also possible to build a learning-based algorithm, that given a query, builds an experience artificially.
% We have tested those two ideas shortly and found them potentially to be applied.

\paragraph{Automatic parameters tuning and optimization}
It empirically shown that \rhcr is highly dependant on  $w$ and $h$ and \exrhcr is also dependent on $\delta$, and $\ell$.
Additionally, it possible to use different $w$ and $h$ for \pbs and \expbs.
To this end, an automatic optimizer that learns the scenario features and suggests parameters is highly relevant and can improve throughput accordingly.

\paragraph{Suggest other \wldfs version}
Instead of execute \pbs as fallback, it possible to use other regions of the expanded PT that outside the sub-tree with width $\ell$.
This idea can be also generalized to \dfs version which can be applied to general search on graphs problems.

% Other \findfb function can be implemented, that reuse previous calculated state from the $\OPEN$ list.
% For example, assign the current search state to other node from the open list that is outside the dead-end sub-tree.
% This will search for a solution in other nodes that already calculated instead of execute \pbs from scratch, and also can be applied in \pbs itself and even other search on graphs problem.




% \paragraph{Learn $b$ dynamically during the search}
% We used \wldfs for improve \expbs with a fixed width limit $b=10$. 
% This parameter affects the solution and performance and its choice is important and should fit the scenario and the PT dimensions. 
% Selecting $b$ that matches the scenario features will reduce additional irrelevant nodes expansion, which equivalent to runtime.
% % Because if $b$ is too large, it may lead to additional irrelevant nodes expansion and consume more runtime, or in better case, avoid unnecessary pruning and find a solution in an area that just disguises itself as a dead-end sub-tree. 
% % On the other hand, when $b$ is too small, the search might prune a solvable direction early or avoid unnecessary expansion.
% It possible to develop method that uses data from the expanded PTs dimensions of \pbs during the experience building process, to learn an optimized $b$ per scenario.



% add next paragraph if there is enough space
% \paragraph{Utilizing working time to improve the EDB} 
% In the problem of lifelong MAPF in real-world, the system is supposed to operate in a huge number of working hours. 
% This time is as an opportunity for EDB improvement (when the offline approach for gaining experience is in use), in our point of view.
% For example, assuming that \expbs works during work hours and the developed maintenance algorithm improve the EDB quality that works after the work hours.
% Such maintenance can improve the quality of the EDB by adding experience from regions in the query space that has long runtime comparing to the average runtime or cleaning some priorities that are founded as over-constrained. \NM{remove?}

% \paragraph{Algorithm selection for \expbs version}
% \NM{add it?}

% \paragraph{Incorporate our algorithmic framework in lifelong planner}
% We mentioned that \pbs performs well as a lifelong MAPF solver according to~\cite{li2021lifelong}, that use bounded horizon (not a new idea,~\cite{silver2005cooperative} already applied it for regular MAPF) planning. In other words, it solves the problem by decomposing it into a sequence of sub-problems, each one is a windowed MAPF instance.
% In addition to integrating \expbs into their solver, we thought about ideas that can be done in this context:
% \begin{itemize}
%     \item \textbf{Transfer experience between subsequent queries:} In the lifelong MAPF algorithm version we discussed, windowed MAPF instances are solved using some parameters that represent the planning horizon, $w$, and time for replanning, $h$. 
%     They used $h=5$, and conclude that a bigger time horizon and bigger replanning factor do not perform better. These insights lead us to think about transferring experience between adjacent windowed instances. 
%     Due to the fact that $h$ is small, instances will be similar according to our metric (each agent moves 5 steps at most), hence, there is a high probability that using the experience from the first windowed instance will reduce runtime in the following one (similar to the results shown in~\ref{sec:feasibility}).
    
%     \item  \textbf{Utilizing working time to improve the EDB:} 
%     In the problem of lifelong MAPF in real-world, the system is supposed to operate in a huge number of working hours. We think of this time as an opportunity for improvement.
%     For example, assuming that \expbs works during work hours and the developed maintenance algorithm improve the EDB quality that works after the work hours.
%     Such maintenance can improve the quality of the EDB by adding experience from regions in the query space that has long runtime comparing to the average runtime or cleaning some priorities that are founded as over-constrained.
    
    
%     \item  \textbf{Parallel calculation of several experiences or solvers version:} One of the \wldfs fallbacks we proposed was using other experiences when the width limit is violated. Similarly, for a big system such as Amazon's warehouses, it is probably optional to run a number of computers in parallel, where each one uses a different experience or algorithm version and the fastest solution will be used.

% \end{itemize}




==> tex/old_algorithmic_framework.tex <==

\section{Algorithmic Background}
In this section we describe two algorithmic components, which we will build upon to design our effective approach for L-MAPF in Sec.~\ref{sec:algorithm}. In particular we describe Priority-Based Search (\pbs) for MAPF, and the Rolling-Horizon Collision Resolution (\rhcr) for L-MAPF. 
% ===================

% \subsubsection{\Castar} Cooperative \astar ~\cite{silver2005cooperative} deals with the MAPF problem with simple \emph{prioritized planning}~\cite{erdmann1987multiple} approach, which is widely used in practice due to its efficiency.
% The agents are ordered by predefined order, and every agent in its turn searches for the shortest path without colliding with the paths of agents with a higher priority that already computed their paths. 
% Technically, the path is calculated for agent w.r.t. paths of agents with higher priorities, which are written into a global reservation table. 

% ===================

% \subsubsection{\whcastar} 
% Windowed Hierarchical Cooperative \astar (\whcastar), which is also introduced in~\cite{silver2005cooperative}, is a bounded-horizon version  of \Castar which also uses an abstract heuristic to improve performance. 
% This algorithm is based on the idea of the Hierarchical \astar algorithm~\cite{holte1996hierarchical}, which improves the heuristic by abstracting the space. 
% In addition, it improves some drawbacks of \Castar by limiting the search with a fixed time window $w$. That means the algorithm searches for a path for an agent that avoids collision with higher priority agents for only the first $w$ timesteps.
% This idea aims to reduce the number of conflicts which therefore expands fewer nodes and runs faster and finds a solution.

% ===================

% \subsubsection{\cbs} Conflict-Based Search (\cbs)~\cite{sharon2015conflict} is  a complete and optimal MAPF solver that forms a two-level search-based algorithm.
% The high-level part of \cbs performs a best-first search on a binary \emph{constraint tree} (CT) that uses the CT nodes costs, which calculated using some objective function. 
% Each high-level node $N \in \text{CT}$ contains a single solution $(N.solution)$ and its cost $(N.cost)$ where a solution satisfies a set of (negative) constraints imposed on the agents $(N.constraints)$. 
% Such a constraint is represented by a tuple $\langle a_i, v, t \rangle$ $(\langle a_i, e, t \rangle)$ and implies that agent $a_i$ is prohibited from occupying vertex $v$ (edge $e$ at time step $t$). 
% A CT node information is generated by the low-level search of \cbs. In the low-level, the algorithm finds the shortest paths, one for each agent, that satisfy all high-level node constraints by using an efficient search algorithm, such as \astar. When this solver is invoked for some agent, it ignores all other agents but considers the constraints from the CT node. Once \cbs has chosen a CT node for expansion, it checks the current solution for conflicts. 
% If the CT node $N$ is conflict-free, then \cbs returns its solution.
% Otherwise, \cbs splits the CT node $N$ on one of the conflicts, 
% % as mentioned in Definition~\ref{def:collisions},
% $\langle a_i, a_j, v, t \rangle$ (or $\langle a_i, a_j, e, t \rangle$ for edge conflicts) by generating two children, each of them inherits the constraints of $N$, and a new constraint that prevents agents $a_i$ $(a_j)$ from being at vertex $v$ (or traverse the edge $e$) at time step $t$. 
% % Fig.~\ref{fig:cbs_sol} visualizes the \cbs search process on the scenario as provided in Fig.~\ref{fig:mapf_graph_solution_visualization}. The agents collide in $v=(2,2)$ at timestep $t=1$, two children CT nodes are generated with the corresponded constraints, the left node generates another collision where the right solves the scenario.
% In addition to being popular algorithms for the MAPF problem, \cbs is also forming an infrastructure for a family of algorithms, that are among the state-of-the-art algorithms. 
% % Each one of the algorithms in that family, suggests an improvement, change, or new approach that is based on \cbs idea for solving MAPF or even other problems.

% ===================

\subsection{Priority-Based Search (\pbs)} 
%Priority-Based Search (\pbs)~\cite{ma2019searching} is a recent approach for MAPF that has been shown to be much faster than the popular \cbs method. Although \pbs does not provide completeness guarantees, it is favorable in large problem instances, or situations where multiple MAPF instances need to be solved rapidly (as in L-MAPF). 

Priority-Based Search (\pbs)~\cite{ma2019searching} is a recent approach for MAPF that has been shown to be orders of magnitudes faster than alternative MAPF solvers. 
This is achieved by foregoing completeness guarantees and taking a \emph{prioritized} approach (to be explained shortly).
The efficiency of \pbs makes it a favorable algorithm to tackle extremely large problem instances, or situations where multiple MAPF instances need to be solved rapidly (as in L-MAPF). 

We now provide an overview of \pbs, and refer the reader to~\cite{ma2019searching} for the full description. %In its core, \pbs has some resemblance to \cbs, in that it 
\pbs performs a bi-level search, where the high-level search explores different priorities between agents, and the low-level search finds agent paths that abide to the priorities. Priorities are used as a coarser and more computationally-efficient alternative to \emph{high-level constraints}, which specify where certain agents cannot be at certain points in time to avoid conflicts (as in \cbs). %We now provide more details about the two levels.  

%However, unlike \cbs which maintains time-location constraints between the agents in the high-level search which specify where certain agents cannot be at certain points in time, \pbs adopt a \emph{prioritized planning}~\cite{erdmann1987multiple} approach.
%In particular, \pbs specifies priorities between agents which are used to resolve conflicts. The low-level of \pbs search aims to find single-agent paths that abide to specific priorities. In contrast to previous work which maintained one specific priority between the agents~\cite{silver2005cooperative}, \pbs explores various priorities through the high-level search. 

%combines ideas between two algorithms: (i) Cooperative \astar (\Castar)~\cite{silver2005cooperative}, which is a simple (possibly incomplete) approach to deal with MAPF through a \emph{prioritization} between agents~\cite{erdmann1987multiple} \KS{Unclear why there are two separate citations here.}\NM{the second one is for "prioritized planning"} \KS{This text is currently quite vague and does not provide meaningful information, so it's hard to understand what is the purpose of the two references}, and (ii) \cbs. 

% \begin{enumerate}

%     \item 
%         Conflict-Based Search (\cbs)~\cite{sharon2015conflict}, which is a known two-level search-based solver that provides completeness and optimality.
        
%         % The high-level part of \cbs performs a best-first search on a binary \emph{constraint tree} (CT), in order to solve collisions. 
%         % The low-level searches for the shortest paths, one for each agent, that satisfies all high-level node constraints by using an efficient search algorithm, such as \astar ~\cite{hart1968formal}.
%         % When this solver is invoked for some agent, it ignores all other agents but considers the constraints from the CT node. 
%         % This search continues iteratively until finding a feasible path for all agents.
    
%     \item %\textbf{\Castar}
%         Cooperative \astar (\Castar)~\cite{silver2005cooperative}, which deals with the MAPF problem with simple \emph{prioritized planning}~\cite{erdmann1987multiple} approach.
%         % which is widely used in practice due to its efficiency.
%         % The agents are ordered by predefined order, and every agent in its turn searches for the shortest path without colliding with the already computed  paths of agents with a higher priority. 
%         % Technically, the path is calculated for agent w.r.t. paths of agents with higher priorities, which are written into a global reservation table. 
% \end{enumerate}

On the high-level search \pbs explores a \emph{priority tree} (PT), where a given node $N$ of PT encodes partial priority ordering $\PREC_N=\{a_{i_1}\prec a_{i'_1}, a_{i_2}\prec a_{i'_2}$, \ldots \}. A priority $a_{i_j}\prec a_{i'_j}$ means that agent $a_{i_j}$ has precedence over agent $a_{i'_j}$ whenever a low-level search is invoked. In addition to the ordering, each PT node maintains single-agent plans that represent the current solution to MAPF (possibly with conflicts). 
\pbs starts the high-level search with the tree root whose priority set is empty, and assigns to each agent its shortest path. Whenever \pbs expands a node $N$, it invokes a low-level search to compute a new set of plans which abide to the priorities $\PREC_N$. If a collision between agents, e.g., $a_i$ and $a_j$, is encountered in the new plans, \pbs generates two child PT nodes $N_1, N_2$ with the updated priorities $\PREC_{N_1}=\PREC_N\cup \{a_i\prec a_j\}, \PREC_{N_2}=\PREC_N\cup \{a_j\prec a_i\}$, respectively. The high-level search expands PT nodes via a depth-first search (\dfs). The high-level search terminates when a feasible solution is a found at some node $N$, or when no more nodes for expansion are remaining, in which case, \pbs declares failure. 

The low-level search of \pbs proceeds in the following manner. For a given PT node $N$, \pbs performs a topological sort of the agents according to $\PREC_N$ from high priority to low, and plans individual-agent paths based on the sorting. 
For a given topological sort $(a'_{1},\ldots, a'_{\eta})$, for some $1\leq \eta\leq k$ (note that agents that do not appear on this list maintain their original plans),  the low level iterates over all $\eta$ agents in the topological sort, and updates their plans such that it does not collide with any higher-priority agents. It then checks whether collisions occur between all the agents combined. 




%is also two-level algorithm, which its low-level is based on prioritized planning, like \Castar. 
%It searches paths for agents considering partial priority ordering, which is given from the high-level node information. 
%The high-level search of \pbs treats collisions by assigning priorities between the colliding pairs of agents.

%his partial priority ordering is incrementally constructed during the high-level search.%\pbs does not store constraints explicitly in the PT nodes but maintains the invariant that, if pair of agents has any priority relation, their paths will not collide. 
%\pbs performs a \emph{depth-first search} (\dfs) to dynamically build a \emph{priority tree} (PT) until a solution is found. 
%Each PT node $N \in \text{PT}$ contains a set of partial priority ordering between couples denoted by $\PREC_N$ and performs the low-level search accordingly. 
%Paths will be first computed for agents with higher priority, and lower-priority agents will use these paths as constraints. 
% Hence, \pbs does not store constraints explicitly in the PT nodes but maintains the invariant that, if pair of agents has any priority relation, their paths will not collide. 
% This invariant means that the priority relation indirectly contains additional information of low-level constraints. 
%When \pbs update paths for agent $a_i$ in PT node $N$, it performs a topological sort for $a_i$ and lower priorities agents $a_j$, according to $\PREC_N$. 
%After $a_i$ path is updated, paths of other agents are also updated, according to the same topological sort, to avoid other collisions.
% This, in turn, can be used in our algorithmic framework as a sparse representation of experience.

% Algorithm~\ref{alg:original_pbs} provides a pseudo-code that details the high-level search of \pbs. 

% Fig.~\ref{fig:pbs_sol} shows an example for \pbs search process on the scenario as provided in Fig.~\ref{fig:mapf_graph_solution_visualization}. The agents collide in $v=(2,2)$ at timestep $t=1$, two children PT nodes are generated with the corresponded priorities, which is $a_1 \prec a_2$ at the right child and $a_1 \prec a_2$ at the left.
% The left child causes another collision that can not be solved (no more priorities can be added and the current state is not a solution). In contrast, the right child calculates the path for the blue agent, which is $a_2$, taking into account the calculated path of $a_1$, and that leads to a solution. This example also demonstrates the advantage of \pbs, which provides a fast solution due to the usage of prioritized planning for MAPF.

% ===================

\subsection{\rhcr} 
Rolling-Horizon Collision Resolution (\rhcr)~\cite{li2021lifelong}, is a promising framework for solving L-MAPF. \rhrc accepts as parameters a time window $w\geq 0$, and a replaning rate $h\leq w$, and decomposes the L-MAPF  problem into a sequence of  W-MAPF queries denoted by $q_1, q_2, \ldots$ that are solved one by one. In particular, after obtaining a W-MAPF plan for a query  $q_i$ with time window $w$, the next $q_{i+1}$ is generated executing the solution plan to $q_{i}$ for $h$ steps, which yields the initial agent locations, and updating the goal locations of agents that finished their task in $q_{i}$ according to the task assigner.   \rhcr employs a simple domain-specific task assigner, which we will use below as well. %We mention that but we it flexible and generalizable for other task assigners. 

Using this framework requires bounded-horizon versions of MAPF solvers as an internal submodule. %such as \whcastar.
Accordingly, several bounded-horizon versions of state-of-the-art MAPF algorithms were developed and used, among which \pbs proved to be the most effective as a W-MAPF solver within \rhcr.  Overall, it was observed that by using a small time window~$w$, and consequently a small replaning rate~$h$, \rhcr can obtain faster solutions than alternative approaches. This, in turn, allows to solve queries containing more agents which, consequently has the potential to improve the system's throughput~\cite{li2021lifelong}. 

%Additionally, among the algorithms tested as infrastructure, \pbs outperform the other.
% In addition, this framework uses a simple domain-specific decoupled task assigner, that can generalize other task assigner and domains.

% \section{Related Work \NM{todo - delete and move to intro}}
% \subsection{Experience in \cbs-like Algorithms}





% \section{Problem Definition}
% Using the MAPF and lifelong MAPF setting as described before, we focus on adopting MAPF solver $\mathbb{S}$ and information from its previous solutions $\calI(q)$ and develop a solver version $\mathbb{S}_{\textsf{exp}}(\calI(q))$, that improves performance and efficiency of solving similar query $\Tilde{q}$ using $\calI(q)$.
% Specifically, We want to use build such a solver that will be used in lifelong MAPF framework in order to increase throughput by improving the agents scalability.
